Noise Flow: Noise Modeling with Conditional Normalizing Flows

Modeling and synthesizing image noise is an important aspect in many computer vision applications. The long-standing additive white Gaussian and heteroscedastic (signal-dependent) noise models widely used in the literature provide only a coarse approximation of real sensor noise. This paper introduces Noise Flow, a powerful and accurate noise model based on recent normalizing flow architectures. Noise Flow combines well-established basic parametric noise models (e.g., signal-dependent noise) with the flexibility and expressiveness of normalizing flow networks. The result is a single, comprehensive, compact noise model containing fewer than 2500 parameters yet able to represent multiple cameras and gain factors. Noise Flow dramatically outperforms existing noise models, with 0.42 nats/pixel improvement over the camera-calibrated noise level functions, which translates to 52% improvement in the likelihood of sampled noise. Noise Flow represents the first serious attempt to go beyond simple parametric models to one that leverages the power of deep learning and data-driven noise distributions.

==> Noise Flow_ Noise Modeling with Conditional Normalizing Flows/fig_camparams.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figs/cam_params.pdf}
        \caption{Camera gain weights\label{fig:cam-params-gain}}
    \end{subfigure}%
    \begin{subfigure}[b]{0.49\columnwidth}
	\centering
    	\raisebox{1mm}{\includegraphics[width=\columnwidth]{figs/cam_beta1_all.pdf}}
        \caption{Camera $\beta_1$ values \label{fig:cam-params-beta1}}
    \end{subfigure}
    \caption{(a) Learned camera-specific weights for the shared gain layer indicates differences in the gain of different cameras. These gains are correlated with the cameras' different values for NLF parameter $\beta_1$ shown in (b). The iPhone and G4 cameras have smaller ranges of ISO values in the SIDD dataset and hence their correlation with the gains is not clear.%
    \vspace{-2mm}}%
    \label{fig:cam-params}%
\end{figure}

==> Noise Flow_ Noise Modeling with Conditional Normalizing Flows/fig_noisesamples.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figs/noise-samples-iso.pdf}%
    \caption{Generated noise samples from (c) Noise Flow are much closer, in terms of marginal KL divergence, to (d) the real samples; compared to (a) Gaussian and (b) camera NLF models. (e) Clean image. Corresponding ISO levels and lighting conditions are on the left.}%
    \label{fig:noise-samples}%
\end{figure}


==> Noise Flow_ Noise Modeling with Conditional Normalizing Flows/fig_sdngainparams.tex <==
\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.49\columnwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figs/sdn_params_exp.pdf}
        \caption{Signal-dependent parameters\label{fig:sdn-params}}
    \end{subfigure}
    \begin{subfigure}[t]{0.49\columnwidth}
    	\centering
    	\includegraphics[width=\columnwidth]{figs/gain_params_exp_iso.pdf}
        \caption{Gain parameters\label{fig:gain-params}}
    \end{subfigure}
    \caption{(a) Signal-dependent noise parameters $\beta_1$ and $\beta_2$ are consistent with the signal-dependent noise model where $\beta_1$ is dominant and $\beta_2$ is much smaller. (b) The gain parameters, in log scale, are consistent with the corresponding ISO levels shown in the legend.\vspace{-3mm}}%
    \label{fig:sdn-and-gain-params}%
\end{figure}

==> Noise Flow_ Noise Modeling with Conditional Normalizing Flows/notation.tex <==
% \newcommand{\obsvar}{\mathcal{Y}}
\newcommand{\obsval}{\mathbf{n}}
\newcommand{\obsvali}{n}
%\newcommand{\obsdensity}{p_\obsvar}
\newcommand{\obsdensity}{p}
\newcommand{\obsdata}{\mathcal{D}}
\newcommand{\obsnum}{M}

\newcommand{\flowvar}{\mathcal{X}}
\newcommand{\flowval}{\mathbf{x}}
\newcommand{\flowvali}{x}
\newcommand{\flowdim}{D}
\newcommand{\flownum}{N}
\newcommand{\flowfunc}{f}
\newcommand{\flowinv}{g}
\newcommand{\flowfuncJ}{\mathbf{J}}
\newcommand{\flowinvJ}{\mathbf{H}}
\newcommand{\flowparams}{\theta}

\newcommand{\basevar}{{\flowvar_0}}
\newcommand{\baseval}{{\flowval_0}}
\newcommand{\baseset}{\mathfrak{X}}
\newcommand{\basedensity}{p_\basevar}
\newcommand{\baseparams}{\phi}

\newcommand{\scalbijection}{h}
\newcommand{\actfunction}{h}

\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\params}{\Theta}
\newcommand{\diag}{\textrm{diag}}

\newcommand{\conv}{\star}
\newcommand{\emult}{\otimes}
\newcommand{\FT}{\mathcal{F}}
\newcommand{\IFT}{\mathcal{IF}}

%\newtheorem{lemma}{Lemma}
\renewcommand{\eg}{e.g.} % as recommended by the copy editor.
\renewcommand{\ie}{i.e.}
\newcommand{\marcus}[1]{ {\color{blue}{\bf Marcus:} #1 } }
\newcommand{\msb}[1]{ {\color{green}{\bf MSB:} #1 } }
\newcommand{\abdo}[1]{ {\color{red}{\bf Abdo:} #1 } }
\newcommand{\comment}[1]{ }

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\cleanim}{\mathbf{I}}
\newcommand{\gcleanim}{\cleanim_{\gain}}
\newcommand{\noisyim}{\mathbf{\Tilde{I}}}
% \newcommand{\noisevar}{\mathbf{y}}
% \newcommand{\noiseval}{y}
\newcommand{\noisevar}{\obsval}
\newcommand{\noiseval}{\obsvali}
\newcommand{\poiscomp}{\alpha}
% \newcommand{\gauscomp}{\gamma}
\newcommand{\gauscomp}{\delta}
\newcommand{\scale}{\mathbf{s}}
%\newcommand{\gain}{\mathrm{g}}
\newcommand{\gain}{\gamma}
\newcommand{\camparam}{\psi}
\newcommand{\camidx}{m}
\newcommand{\camfunc}{f_\camparam}
\newcommand{\ISO}{\textrm{ISO}}

\newcommand{\trainset}{\obsdata_\mathrm{r}}
\newcommand{\testset}{\obsdata_\mathrm{s}}
\newcommand{\KL}{D_{KL}}
\newcommand{\sampdata}{\mathcal{S}}
\newcommand{\nll}{\mathit{NLL}}

% commands
% text colors
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
%
\setlength\delimitershortfall{0pt}
% cell colors
\newcommand{\gcl}{\cellcolor{green!25}}
\newcommand{\bcl}{\cellcolor{blue!25}}
\newcommand{\rcl}{\cellcolor{red!25}}
% superscripts
\newcommand{\tss}[1]{\textsuperscript{#1}}
% ranking colors
\newcommand{\arnk}[1]{\gcl ~\textbf{#1}}
\newcommand{\brnk}[1]{\bcl ~#1}
\newcommand{\crnk}[1]{\rcl ~#1}
\newcommand{\aarnk}[1]{\gcl\fontseries{b}\selectfont{#1}}

\newcommand{\parag}[1]{\noindent\textbf{#1}~~}
\newcommand{\paragskip}[1]{\medskip\noindent\textbf{#1}~~}

